Quantum Complexity of Nonlocal Field Theories

Entanglement entropy for nonlocal field theories displays a universal ``volume law" scaling \cite{Barbon:2008ut, Karczmarek:2013xxa, Shiba:2013jja, Pang:2014tpa} as opposed to the ``area law" scaling for local field theories. The aim of this work is to determine whether complexity displays any such an universal scaling laws. The field theories considered here are obtained by deforming $\mathcal{N}=4$ SYM theory by higher dimension operators introducing nonlocality, namely a dipole deformation and noncommutativity (NCSYM) by turning on world volume Kalb-Ramond $B$ field. The dual gravity backgrounds have a running dilaton, in addition to the $B$-field background, which alter AdS asymptotics. Our results capture nonlocality in the hyperscaling behavior for complexity. We also compute the subregion complexity which display phase transitions in the nonlocal field theories with the transition point being the same as that for the phase transition of entanglement entropy \cite{Karczmarek:2013xxa}. These new results dovetail nicely with our findings from our previous works \cite{Chakraborty:2020fpt, Katoch:2022hdf, Bhattacharyya:2022ren} on other lower dimensional nonlocal field theories such as little string theories (LSTs) and warped conformal field theories (WCFTs).

==> Subregion_Complexity_Sai.tex <==
% \section{Non Commutative SYM-complexity}
% Since we did not find any non-commutativity in the above, we will find the Complexity in a more general context. Let the metric be as follows,
% \begin{align}
%     ds^2=R^2u^2(-f(u)dt^2+g(u)dx^2+k(u)dy^2+i(u)dz^2)+R^2\frac{du^2}{u^2}+R^2d\Omega_5^2
% \end{align}
% Here $f(u),g(u),i(u),k(u)$ are just some functions of u, we will replace them with either 1 or $h(u)$, depending on which coordinates have non-commutativity.
% Space like hyper surface is given by $t=t(u)$. This gives the metric as,
% \begin{align}
% ds^2=R^2u^2(g(u)dx^2+k(u)dy^2+i(u)dz^2)+R^2\frac{du^2}{u^2}\left(1-u^4t'(u)f(u)\right)+R^2d\Omega_5^2
% \end{align}
% Volume is given by,
% \begin{align}
%     V&=\int d^9\sigma e^{-2(\phi-\phi_0)}\sqrt{|g_{\mu\nu}|}\\
%     &=R^9\omega_5 L^3\int du \frac{u^2}{h(u)}\sqrt{g(u)k(u) i(u)}\sqrt{1-u^4t'^2(u)f(u)}
% \end{align}
% Since, $u>0$ and $f(u)>0$(since it is either 1 or $h(u)$), the maximum of the function is when we have $t'(u)=0$. This gives,
% \begin{align}
%     V&=R^9\omega_5 L^3\int du \frac{u^2}{h(u)}\sqrt{g(u)k(u) i(u)}
% \end{align}
% \subsection{Anisotropic cases}
% If we consider the non-commutativity in only $t$, we have $f(u)=h(u)$ and $g(u)=k(u)=i(u)=1$. This gives,
% \begin{align}
%     V_t&=R^9\omega_5 L^3\int_{0}^{u_B} du\frac{u^2}{h(u)}\\
%     V_t&=R^9\omega_5 L^3\left(\frac{u_B^3}{3}+\frac{a^4u_B^7}{7}\right)
% \end{align}
% We read $V_t$ as "$V$ when non commutativity is only in $t$".\\
% Similarly if we consider the non-commutativity in either $x/y/z$, we get the same answer. For this we can see that one of $g(u)/k(u)/i(u)=h(u)$ and others are equal to one. This gives,
% \begin{align}
%     V_{x/y/z}&=R^9\omega_5 L^3\int_{0}^{u_B} du\frac{u^2}{\sqrt{h(u)}}\\
%     V_{x/y/z}&=R^9\omega_5 L^3\left(\frac{u_B^3}{3} {}_2F_1\left[-\frac{1}{2},\frac{3}{4},\frac{7}{4},-a^4u_B^4\right]\right)
% \end{align}
% Similarly for other cases we get the following,
% \begin{align}
%     V_{xy/yz/zx}&=R^9\omega_5^2L^3\frac{u_B^3}{3}\\
%     V_{t,x/y/z}&=R^9\omega_5 L^3\left(\frac{u_B^3}{3} {}_2F_1\left[-\frac{1}{2},\frac{3}{4},\frac{7}{4},-a^4u_B^4\right]\right)\\
%     V_{t,x,y/z}&=R^9\omega_5^2L^3\frac{u_B^3}{3}\\
%     V_{x,y,z}&=R^9\omega_5 L^3\left(\frac{u_B^3}{3} {}_2F_1\left[\frac{1}{2},\frac{3}{4},\frac{7}{4},-a^4u_B^4\right]\right)\\
% \end{align}
% \subsection{Isotropic case}
% For isotropic case, we have non-commutativity for $t,x,y,z$, which has $g(u)=k(u)=i(u)=f(u)=h(u)$. This gives,
% \begin{align}
%     V_{t,x,y,z}=&R^9\omega_5L^3\int_{0}^{u_B} u^2 \sqrt{h(u)}\\
%     &=R^9\omega_5L^3\left(\frac{u_B^3}{3} {}_2F_1\left[\frac{1}{2},\frac{3}{4},\frac{7}{4},-a^4u_B^4\right]\right)
% \end{align}
% \textbf{In summary,}
% \begin{align}
%     V_{x/y/z}=V_{t,x/y/z}&=R^9\omega_5L^3\left(\frac{u_B^3}{3} {}_2F_1\left[\frac{1}{2},\frac{3}{4},\frac{7}{4},-a^4u_B^4\right]\right)\\
%     V_{xy/yz/zx}=V_{t,x,y/z}=V_{t,x,z/y}=V_{t,z,x/y}&=R^9\omega_5L^3 \frac{u_B^3}{3}\\
%     V_t&=R^9\omega_5L^3\left(\frac{u_B^3}{3}+\frac{a^4u_B^7}{7}\right)\\
%     V_{t,x,y,z}=V_{x,y,z}&=R^9\omega_5 L^3\left(\frac{u_B^3}{3} {}_2F_1\left[\frac{1}{2},\frac{3}{4},\frac{7}{4},-a^4u_B^4\right]\right)
% \end{align}
% We see that only in eq(56), we dont see a non-commutative parameter due to the dimensional accident. But for the others, we can see the effect of non-commutative parameter.\\
\subsection{Isotropic case}
The metric in the paper suggested (by \href{https://inspirehep.net/literature/526906}{Li Ling, Shi Wu }(Eq.2.20)), is given as,
\begin{align}
    ds^2_E &=l^2u^{-2}\Phi^{8/3}du^2+l^2u^2\Phi^{2/3}(-dt^2+dx_1^2+dx_2^2+dx_3^2)
\end{align}
When we take $t=t(u)$, the deduced metric is given as,
\begin{align}
    dh^2&=l^2\Phi^{2/3}\left(\frac{\Phi^2}{u^2}-u^2t'^2(u)\right)du^2+l^2u^2\Phi^{2/3}(d\rho^2+\rho^2d\theta^2+\rho^2 sin^2(\theta)d\phi^2)
\end{align}
Here we take $\rho$ as the radial coordinate and $u$ as the  holographic coordinate. We have $|g_{\mu\nu}|
=l^8u^8\Phi^{4/3}\rho^2sin(\theta)\sqrt{\frac{\Phi^2}{u^4}-t'^2(u)}$. The volume is maximum at $t'(u)=0$, and hence we have the volume as, 
\begin{align}
    V&=\int du\ d\rho \ d\theta \ d\phi \  l^4u^4 \Phi^{4/3}\rho^2 sin(\theta)\sqrt{\frac{\Phi^2}{u^4}-t'^2(u)}\\
    &=4\pi l^4 \int_{0}^{R}d\rho \ \rho^2\int_{0}^{u_B}du \ u^2\Phi^{7/3}\\
    &=\frac{4\pi l^4 R^3}{3}\int_{0}^{u_B} du \ u^2\Phi^{7/3}
\end{align}
Let's define dimensionless quantities as $a u_B=\alpha$, $Ru_B=R_B$ and $\tilde{u}=u/u_B$. Using these we have the Volume as,

\begin{align}
    V&=\frac{4\pi l^4R^3u_B^3}{3}\int_0^1d\tilde{u} \ \tilde{u} (1+\alpha^4 \tilde{u}^4)^{7/3}\\
    &=\frac{2\pi l^4R^3u_B^3}{3}\ {}_2F_1\left[\frac{-7}{3},\frac{1}{2},\frac{3}{2},-\alpha^4\right]\\
    C_V(AdS)&=\frac{2\pi l^3R_B^3}{3G_N^{(5)}}\label{eqn:47}
\end{align}
eq  \ref{eqn:47} matches with the eq (10) of \href{https://arxiv.org/pdf/1612.05439}{Reynolds and ross paper} when we taks $\alpha=0$ which is pure AdS case.\color{red} 
     But the $\epsilon$ that they have is $1/u_B$ here and they used $\epsilon$ as the lower limit for the integration and the upper limit is Infinity.\\ 
\color{black}We can have two limits, one is near AdS and other is non-commutative region. The near AdS expansion is when $au_B<<1$ i.e. when $\alpha<<1$. So the volume is,
\begin{align}
    V&=\frac{2\pi l^4R^3u_B^3}{3} \left(1+\frac{7\alpha^4}{9}+\frac{14\alpha^8}{45}+O[\alpha^{11}]\right)
\end{align}
Similarly for the non-commutative region we have $au_B>>1$ i.e. $\alpha>>1$. So the volume will be,
\begin{align}
    V&=\frac{2\pi l^4R^3u_B^3}{3}\left(\frac{3 \alpha ^{28/3}}{17}+\frac{7 \alpha ^{16/3}}{11}+\frac{14 \alpha ^{4/3}}{15}+O\left[\frac{1}{\alpha^2}\right]\right)=\frac{2\pi l^4R^3u_B^3\alpha^{28/3}}{17}\left(1+O\left[\frac{1}{\alpha^4}\right]\right)
\end{align}
If we take the leading order in $\alpha$ and $\beta=a/R$, we have the scaling law as,
\begin{align}
    V&=\frac{2\pi l^4}{17}\left(\beta^{28/3}\times u_B^{37/3}\times R^{37/3}\right)\\
    V&\propto u_B^{37/3} \times R^{37/3}\times \beta^{28/3}\\
    V&\propto  u_b^{37/3}\times R^{3}\times a^{28/3}
\end{align}
Now, let's calculate the sub region complexity, we assume that it is cubical for simplicity. The metric is given by (we take $z=1/r$) and $\Phi(z)=(1+\frac{a^4}{z^4})^{1/2}$,
\begin{align}
    ds^2&=l^2\Phi^{8/3}\frac{dz^2}{z^2}+l^2\frac{l^2}{z^2}\Phi^{2/3}(dx_1^2+dx_2^2+dx_3^2)=\frac{l^2}{z^2}\Phi^{2/3}(\phi^{2}dz^2+dx_1^2+dx_2^2+dx_3^2)\label{45}
\end{align}
We restrict the values as $-b/2\leq x_1\leq b/2$, $-L/2<x_2,x_3<L/2$. We take $z=z(x_1)$. This gives,
\begin{align}
    ds^2&=\frac{l^2}{z^2}\Phi^{2/3}\left(1+\Phi^2z'^2\right)dx_1^2+l^2r^2\Phi^{2/3}(dx_2^2+dx_3^2)
\end{align}
The area is given as,
\begin{align}
    A&=\int \frac{l^3}{z^3}\Phi\sqrt{1+\Phi^2z'^2}dx_1dx_2dx_3\\
    &=L^2l^3\int_{-b/2}^{b/2} \frac{1}{z^3}\Phi\sqrt{1+\Phi^2z'^2}dx_1
\end{align}
We can take the lagrangian as,
\begin{align}
    \mathcal{L}&=\frac{1}{z^3}\Phi\sqrt{1+\Phi^2z'^2}
\end{align}
Since, the Lagrangian is not explicitly dependent on $x_1$. We can take the Hamiltonian as,
\begin{align}
    H&=z'\frac{\partial \mathcal{L}}{\partial z'}-\mathcal{L}\\
    H&= \frac{-\Phi}{z^3\sqrt{1+\Phi^2z'^2}}
\end{align}
We can evaluate the hamiltonian using the boundary conditions at the turning point $z_*$ occuring is $x_1=0$ and $z'(x_1)=0$. So, the Hamiltonian at this point is given as $H(z_*)=-z_*^3\Phi_*$. This gives,
\begin{align}
    z'&=\frac{1}{\Phi}\sqrt{\left(\frac{\Phi}{\Phi_*}\frac{z_*^3}{z^3}\right)^2-1}\\
    \frac{dz}{dx_1}&=\frac{1}{\Phi}\sqrt{\left(\frac{\Phi}{\Phi_*}\frac{z_*^3}{z^3}\right)^2-1}\\
    \int_{0}^{b/2}dx_1&=\int_{z_*}^{z_B}\frac{\Phi}{\sqrt{\left(\frac{\Phi}{\Phi_*}\frac{z_*^3}{z^3}\right)^2-1}}\\
    b&= 2 \int_{z_*}^{z_B}\frac{\Phi}{\sqrt{\left(\frac{\Phi}{\Phi_*}\frac{z_*^3}{z^3}\right)^2-1}}
\end{align}
Using the above condition, we can get the Area as,
\begin{align}
    A&=L^2l^3\int \frac{\Phi}{z^3}\sqrt{1+\Phi^2 z'^2}dx_1\\
    A&=L^2l^3\int_{z_*}^{z_B}\frac{\Phi^3}{\sqrt{\Phi^2z_*^6-\Phi_*^2z^6}}\left(\frac{z_*}{z}\right)^3dz
\end{align}
The above is also not integrable until we take the AdS limit and $ar_B>>1$. So we take the AdS case and check our results with the eq(7.4) of \href{https://arxiv.org/pdf/hep-th/0605073}{paper} . If $a=0$, we have $\Phi=1$, so the area will be,
\begin{align}
    A&=L^2l^3\int_{z_*}^{z_B}\frac{1}{\sqrt{z_*^6-z^6}}\left(\frac{z_*}{z}\right)^3dz\\
    &=\frac{L^2l^3}{6}\left(\frac{\sqrt{\pi}\Gamma(-\frac{1}{3})}{z_*^2\Gamma(\frac{1}{6})}+\frac{3{}_2F_1[-\frac{1}{3},\frac{1}{2},\frac{2}{3},\left(\frac{z_b}{z_*}\right)^6]}{z_b^2}\right)
\end{align}
Now we calculate the volume for the metric (\ref{45})
\begin{align}
    V&=\int \sqrt{|g_{\mu\nu}|}dzdx_1dx_2dx_3\\
    &=L^2\int_{z_*}^{z_B} l^4r^2\Phi^{7/3}dr \int_{0}^{L/2} dx_1\\
    V&=L^2l^4\int_{r_*}^{r_B}r^2\Phi^{7/3}dr\int_{r_*}^{r}\frac{\Phi(\tilde{r})d\tilde{r}}{(\tilde{r})^2\sqrt{\left(\frac{{\tilde{r}}^3\Phi}{r_*^3\Phi_*}\right)^2-1}}
\end{align}
The above integral is also not integrable until we take limiting conditions. By numerical integration with the values $a=10^{-7}, r_B=10^{8}$, we have the following graph,
\begin{figure}[H]
    \centering
    \includegraphics[width=0.3\linewidth]{images_volume_complexity/LogVvsLogl_Isotropic.jpg}
    \hfill\includegraphics[width=0.3\linewidth]{images_volume_complexity/LogVvsLogl_Isotropic_log.jpg}
    \label{fig:enter-label}
\end{figure}
Instead of taking a cuboidal surface, we can take a spherical subregion with spherical symmetry. This would have the metric as,
\begin{align}
    ds^2=\frac{l^2}{z^2}\Phi^{2/3}(\phi^{2}dz^2+dx_1^2+dx_2^2+dx_3^2)=\frac{l^2}{z^2}\Phi^{2/3}(\phi^{2}dz^2+dr^2+r^2d\Omega_2^2)
\end{align}
We take $r=r(z)$, so we will have the area as,
\begin{align}
    A=4\pi l^3\int_{0}^{z_0}\frac{dz}{z^3}\Phi r^2\sqrt{\Phi^2+r'^2}
\end{align}
So we would have the Lagrangian as,
\begin{align}
    \mathcal{L}=\frac{1}{z^3}\Phi r^2\sqrt{\Phi^2+r'^2}
\end{align}
After performing variational analysis to find the EOM, we have the second order DE with the boundary conditions as $r(z_0)=0, r'(z_0)=\infty$ as,
\begin{align}
    r''-\frac{2\left(1+\frac{a^4}{z^4}+r'^2\right)}{r}-\frac{\left(5a^4z^3+3z^7\right)r'^3}{(a^4+z^4)^2}-\frac{3r'}{z}=0
\end{align}
If we take the AdS case we have the DE as,
\begin{align}
    r''-\frac{2(1+r'^2)}{r}-\frac{3r'^3}{2}-\frac{3r'}{2}=0
\end{align}
The solution for this DE is $r^2+z^2=b^2$, this exactly matches with the eq(7.8) of \href{https://arxiv.org/pdf/hep-th/0605073}{paper}. 
% We can solve the above DE perturbatively in $\epsilon=a^4$,
% \begin{align}
%     r(z)&=r_0(z)+\epsilon r_1(z)+\dots\\
%     r(z)&=\sqrt{b^2-z^2}-a^4 \left(\frac{\sqrt{-\left(b^2-z^2\right)^2}+6 b^2 z^2 \left(2 c_2 \sqrt{z^2-b^2}+u_{*1}\right)-6 z^4 \left(c_2 \sqrt{z^2-b^2}+u_{*1}\right)}{6 z^2 \left(z^2-b^2\right)^{3/2}}\right)+\dots
% \end{align}
Here the sub region length is given as,
\begin{align}
    \int_0^{R}dr \  r(z)&=\int_0^{z_0} dz\  (\text{solution of the DE})\\
    R&=\int_0^{z_0}dz\  (\text{solution of the DE})
\end{align}
The volume is given by,
\begin{align}
    V&=4\pi l^4 \int_{0}^{z_0} dz\  \frac{1}{z^4}\Phi^{7/3}\int dr\  r^2\\
    V&=4\pi l^4 \int_{0}^{z_0} dz\  \frac{1}{z^4}\Phi^{7/3} \frac{r(z)^3}{3}
\end{align}
The plots for the Area and the volume complexity are given as follows,
\begin{figure}[H]
    \centering
    \includegraphics[width=0.4\linewidth]{isotropic_complexity_images/a2_area_sublen.jpg}
    \hfill\includegraphics[width=0.4\linewidth]{isotropic_complexity_images/a2_vol_sublen.jpg}
    \label{fig:enter-label}
\end{figure}
The slopes for the above for different values of a are,
\begin{table}[H]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    a & Slope in Area & Slope in Volume\\
    \hline
     0 & 2.4   & 3\\
     \hline
    $10^{-2}$ & 2.6, 1  &3\\
    \hline
    $10^{2}$ & 2.5, 1   &3\\
    \hline
    $10^{4}$ &  2.5, 1 & 3 \\
    \hline
    $10^{6}$&  2.5, 1 & 3 \\ 
    \hline
    $10^{8}$&  2.7, 1 & 3 \\ 
    \hline
    \end{tabular}
    \label{tab:my_label}
\end{table}
\section{Sub-Region Complexity-Non Isotropic case}
To find the sub-region complexity, we restrict the values of x as:
\begin{equation}
    -\frac{l}{2} < x < \frac{l}{2} \quad -\frac{W}{2}<y,z<\frac{W}{2} 
\end{equation}
For the co-dimensional 2 surface we take $u=u(x)$. This gives,
\begin{align}
    ds^2&=R^2 u^2 h(u)(dx^2+dy^2)+R^2 u^2dz^2+R^2\Omega_5^2+R^2 \frac{du^2}{u^2}\\
    d\gamma^2&=R^2 u^2(x)h(u)dy^2+R^2u^2(x)dz^2+R^2u^2(x)h(u)dx^2+R^2\frac{(u'(x))^2}{u^2(x)}dx^2\\
    d\gamma^2&=R^2 u^2(x)h(u)dy^2+R^2u^2(x)dz^2+R^2u^2(x)dx^2\left(h(u)+\frac{(u'(x))^2}{u^2(x)}\right)
\end{align}
The Area is given by
\begin{align}
    A&=\int e^{-2(\phi-\phi_0)}\sqrt{|\tilde{g}_{\mu\nu}|}dx dy dz \\
    &=\int e^{-2(\phi-\phi_0)}\sqrt{R^8u^6h(u)[h(u)+\frac{(u'(x))^2}{u^4(x)}]}\ dx \ dy\ dz\ d\Omega_5^2\\
    &=R^4u^3\int e^{-2(\phi-\phi_0)}h(u) \sqrt{1+\frac{(u'(x))^2}{u^4(x)h(u)}}\ dx \ dy\ dz\ d\Omega_5^2\\
    &=R^4u^3\int_{-W/2}^{W/2}dy\int_{-W/2}^{W/2}dz\int d\Omega_5\int_{-l/2}^{l/2} e^{-2(\phi-\phi_0)}h(u) \sqrt{1+\frac{(u'(x))^2}{u^4(x)h(u)}}\ dx \\
    A&= R^8\omega_5\times W^2\times \int_{-l/2}^{l/2}u^3(x)\sqrt{1+\frac{(u'(x))^2}{u^4(x)h(u)}}dx
\end{align}

To extremize the area we construct the Lagrangian as follows,
\begin{align}
    L&=u^3(x)\sqrt{1+\frac{(u'(x))^2}{u^4(x)h(u)}}
\end{align}
Instead of finding the E.O.M and getting the $u'(x)$, we can construct the Hamilton and use turning point to find $u'(x)$ as follows,
\begin{align}
    H&=u'(x)\frac{\partial}{\partial u'}(L)-L\\
    &= u'(x)\frac{\partial}{\partial u'}\left(u^3(x)\sqrt{1+\frac{(u'(x))^2}{u^4(x)h(u)}}\right)-\left(u^3(x)\sqrt{1+\frac{(u'(x))^2}{u^4(x)h(u)}}\right)\\
    &=-\frac{u^3(x)}{\sqrt{1+\frac{u'^2(x)}{u^4(x) h(u)}}}
\end{align}
We take the turning point as $u_*$ at $x=0$ and $u'(x)=0$, this would give the Hamiltonian as $H(u_*)=-u_*^3$. From (13), we can write $u'(x)$ as,
\begin{align}
    -u_*^3&=-\frac{u^3(x)}{\sqrt{1+\frac{u'^2(x)}{u^4(x) h(u)}}}\\
    \left(\frac{u(x)}{u_*}\right)^6&=1+\frac{u'^2(x)}{u^4(x) h(u)}\\
    (u'(x))^2&=u^4(x)h(u)\left(\frac{u(x)}{u_*}\right)^6-1\\
     u'(x)&=u^2(x)\sqrt{h(u)}\sqrt{\left(\frac{u(x)}{u_*}\right)^6-1}\\
     u'(x)&=\frac{u^2(x)\sqrt{h(u)}\sqrt{u^6(x)-u_*^6}}{u_*^3}\label{udash}
\end{align}
The calculation done by  \href{https://arxiv.org/pdf/1307.3517}{Rabideau} might be as follows. This assumes that the solution, $u$, is near $u_*$.First we take eq \ref{udash}. And we write that in dimensionless parameters, $t=\frac{u}{u_*}$ and $\alpha_*=a u_*$ , as follows,
\begin{align}
    t'(x)&=\frac{u_*t^2\sqrt{t^6-1}}{\sqrt{1+\alpha_*^4t^4}}
\end{align}
Now we expand t as, here t is dimensionless, $t=1+\epsilon+\epsilon^2+\dots$. This would give,
\begin{align}
    t^2\approx 1+2x, \quad \sqrt{t^6-1}\approx \sqrt{6\epsilon}, \quad \frac{1}{\sqrt{1+\alpha^4t^4}}\approx\frac{1}{\sqrt{1+\alpha^4}}
\end{align}
Here we only took until the order of $\epsilon$ and all the higher orders of $\epsilon$ are neglected. So we have,
\begin{align}
    \frac{d(1+\epsilon)}{dx}&=\frac{u_*\sqrt{6\epsilon}}{\sqrt{1+\alpha^4}}\\
    \frac{d\epsilon}{\sqrt{\epsilon}}&=\frac{u_*\sqrt{6}}{\sqrt{1+\alpha^4}}dx\\
    2\sqrt{\epsilon(x)}&=\frac{u_*\sqrt{6}}{\sqrt{1+\alpha^4}}x\\
    \epsilon(x)&=\frac{3u_*^2}{2(1+\alpha^4)}x^2\\
    \implies \frac{u}{u_*}&=1+\epsilon(x)+O[\epsilon^2]=1+\frac{3u_*^2}{2(1+\alpha^4)}x^2+O[\epsilon^2]\\
    u&=u_*+\frac{3u_*^3}{2(1+\alpha^4)}x^2+O(\epsilon^2 u_*)\\
    \implies u_b-u_*&=\frac{3u_*^3}{2(1+a^4u_*^4)}\left(\frac{l}{2}\right)^2+O[l^4]
\end{align}
Now we solve for $u(x)$,
\begin{align}
    \frac{d}{dx}(u(x))&=\frac{u^2(x)\sqrt{h(u)}\sqrt{u^6(x)-u_*^6}}{u_*^3}\\
    \int_{0}^{l/2}dx&=u_*^3\int_{u_*}^{u_B}\frac{du}{u^2(x)\sqrt{h(u)}\sqrt{u^6(x)-u_*^6}}\\
    l&=2 u_*^3\int_{u_*}^{u_B}\frac{du}{u^2(x)\sqrt{h(u)}\sqrt{u^6(x)-u_*^6}}\label{exactl}
\end{align}
We have three different lengths parameters, subregion length $l$, non-commutative parameter $a$, lattice spacing $1/u_b$.With these three parameters we can mathematically have 6 different possibilities,
\begin{align}
    &l\gg \frac{1}{u_b}\gg a, \quad l\gg a\gg \frac{1}{u_b}\\
    &a\gg l\gg \frac{1}{u_b}, \quad a\gg \frac{1}{u_b}\gg l\\
    &\frac{1}{u_b}\gg l \gg a, \quad \frac{1}{u_b}\gg a\gg l
\end{align}
But not all of them are physically meaningful, because the lattice spacing $1/u_b$ should be the lowest length scale as any other quantity being less than that would not be significant. The physically meaningful solutions are,
\begin{align}
\quad  l\gg a\gg \frac{1}{u_b}\ \ \text{(Near AdS region)},\quad
    \ \ a\gg l\gg \frac{1}{u_b} \text{(Far from AdS region)}
\end{align}
If we define $\overline{a}=a/l$, $x_b=l u_b$, these will be,
\begin{align}
    1\gg \overline{a}\gg \frac{1}{x_b},\quad
    \overline{a}\gg 1\gg \frac{1}{x_b},
\end{align}
\subsubsection{Near AdS Case}
First we take the near AdS case, which has the hierarchy as, $1\gg \frac{1}{x_b} \gg \overline{a}$.  In this case, we can rewrite the integral eq (\ref{exactl}) in terms of redefined variables and expand in $\overline{a}$ as,
\begin{align}
    1&=2x_*^3\int_{x_*}^{x_b}\frac{dx\sqrt{1+\bar{a}^4 x^4}}{x^2\sqrt{x^6-x_*^6}}\\
    x_*&=2x_*^4\int_{x_*}^{x_b}\frac{dx\sqrt{1+\bar{a}^4 x^4}}{x^2\sqrt{x^6-x_*^6}}\\
    x_*&=\int_{x_*}^{x_b}\frac{2x_*^4}{x^2 \sqrt{x^6-x_*^6}}+\frac{2\overline{a}^4 x^2x_*^4}{2 \sqrt{x^6-x_*^6}}+O(\overline{a}^8)\\
    x_*&=\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}-\frac{x_*^4}{2 x_b^4} \, _2F_1\left(\frac{1}{2},\frac{2}{3};\frac{5}{3};\frac{x_*^6}{x_b^6}\right)+\frac{1}{6} \overline{a}^4 \tanh ^{-1}\left(\frac{\sqrt{x_b^6-x_*^6}}{x_b^3}\right)\\
    &\hspace{2cm}+\frac{1}{48} \overline{a}^8 x_*^4 \left(-3 x_b^4 \, _2F_1\left(-\frac{2}{3},\frac{1}{2};\frac{1}{3};\frac{x_*^6}{x_b^6}\right)-\frac{2 \sqrt{\pi } x_*^4 \Gamma \left(-\frac{2}{3}\right)}{\Gamma \left(-\frac{1}{6}\right)}\right)+O[\overline{a}^{12}]
    % x_{*0}&=\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}-\frac{x_*^4 \, _2F_1\left(\frac{1}{2},\frac{2}{3};\frac{5}{3};\frac{x_*^6}{x_b^6}\right)}{2 x_b^4}\\
    % x_{*0}&=\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}-O\left(\frac{x_*^4}{x_b^4}\right)\\
    % x_{*1}&=\frac{1}{3} \overline{a}^4 x_*^4 \log \left(\frac{2}{k^3}\right)+O\left(\frac{x_*}{x_b}\right)^5\\
    % \implies x_*&=\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}+\frac{1}{3} \overline{a}^4 x_*^4 \log \left(\frac{2x_b^3}{x_*^3}\right)+O\left(\frac{x_*}{x_b}\right)^5
\end{align}
Here if we take the limit such that $x_*/x_b\ll 1$ and if we expand this around $0$, we have an expansion 
\begin{align}
    x_*\sim & \frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}+\frac{1}{3} \overline{a}^4 x_*^4 \log \left(\frac{2x_b^3}{x_*^3}\right)-\frac{1}{48} \overline{a}^8 x_*^4 \left(3 x_b^4+\frac{2 \sqrt{\pi } x_*^4 \Gamma \left(-\frac{2}{3}\right)}{\Gamma \left(-\frac{1}{6}\right)}\right)+O[a^{12}]\\
    u_*\sim &\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{l \Gamma \left(\frac{1}{6}\right)}-\frac{a^4 u_*^4}{l} \log \left(\frac{u_*}{\sqrt[3]{2} u_b}\right)+O(a^8)
\end{align}
Now we write $u_*$ in terms of l, so that we can substitute this in $C_V$ to get the complexity in terms of sub region length.
\begin{align}\label{uStarinlnearads}
    u_*&=\frac{1}{l}\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{ \Gamma \left(\frac{1}{6}\right)}-\frac{a^4}{l^5}\frac{ 16 \pi ^2  \Gamma \left(\frac{2}{3}\right)^4}{ \Gamma \left(\frac{1}{6}\right)^4} \log \left(\frac{1}{l u_b}\frac{2^{2/3} \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}-\frac{8\ 2^{2/3} \pi ^2 a^4 \Gamma \left(\frac{2}{3}\right)^4 \log \left(\frac{2^{2/3} \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{l u_b \Gamma \left(\frac{1}{6}\right)}\right)}{l^5 u_b \Gamma \left(\frac{1}{6}\right)^4}\right)\\
    u_*&=\frac{1}{l}\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{ \Gamma \left(\frac{1}{6}\right)}-\frac{a^4}{l^5}\frac{ 16 \pi ^2  \Gamma \left(\frac{2}{3}\right)^4}{ \Gamma \left(\frac{1}{6}\right)^4} \log\left(\frac{1}{l u_b}\frac{2^{2/3} \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}\right)\log\left(1-\frac{8 \pi ^{3/2} a^4 \Gamma \left(\frac{2}{3}\right)^3 \log \left(\frac{2^{2/3} \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{l u_b \Gamma \left(\frac{1}{6}\right)}\right)}{l^4 \Gamma \left(\frac{1}{6}\right)^3}\right)\\
    u_*&=\frac{1}{l}\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{ \Gamma \left(\frac{1}{6}\right)}-\frac{a^4}{l^5}\frac{ 16 \pi ^2  \Gamma \left(\frac{2}{3}\right)^4}{ \Gamma \left(\frac{1}{6}\right)^4} \log\left(\frac{1}{l u_b}\frac{2^{2/3} \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}\right)\left(-\frac{a^4}{l^4}\frac{8 \pi ^{3/2} \Gamma \left(\frac{2}{3}\right)^3 \log \left(\frac{2^{2/3} \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{l u_b \Gamma \left(\frac{1}{6}\right)}\right)}{\Gamma \left(\frac{1}{6}\right)^3}+O\left(\frac{a^8}{l^8}\right)\right)\\
    u_*&=\frac{1}{l}\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{ \Gamma \left(\frac{1}{6}\right)}+\frac{a^8}{l^9}\frac{128 \pi ^{7/2}  \Gamma \left(\frac{2}{3}\right)^7}{ \Gamma \left(\frac{1}{6}\right)^7} \log ^2\left(\frac{2^{2/3} \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{l u_b \Gamma \left(\frac{1}{6}\right)}\right)+O\left(a^{12}\right)
\end{align}
% \color{red}So here if we take the pure AdS case i.e. when $\bar{a}=0$, the pure AdS solution will also be a series expansion, which defies the reason (so that we can avoid Hypergeometric functions and get the exact answer) why we are doing the $x_*$ expansion first, instead of $\bar{a}$ expansion.\color{black}
% \begin{align}
%     \frac{1}{2x_*^3}&=\int_{x_*}^{x_b} dx\left(\frac{1}{x^5}+\frac{x_*^6 }{2x^{11}}+O\left(\frac{x_*^{12}}{x^{12}}\right)\right)
% \end{align}
% \subsubsection{Near AdS Expansion}
% For the near AdS case the hierarchy would be $l\gg1/u_B\gg a $. By defining dimensionless quantities $u/u_B=t^{1/3}$,$\alpha=au_B$ and $\overline{u}_*=u_*/u_B$, we can expand (\ref{exactl}) in $\alpha$ first and then take the series expansion of $\overline{u}_*$ near 0. This is because $\overline{u}_*$ is in the limit of integration, taking series expansion of $\overline{u}_*$ near 0 first needs careful consideration of the limits of integration. In terms of dimensionless parameters, the hiearchy is $\bar{l}\gg 1 \gg \alpha $  
% % {\color{blue}{(in powers of which dimensionless parameter and why e.g. there is no clarification as to why first expand in $\alpha$ and only then in $\overline{u}_*$)}}.
% \begin{align}
%     lu_*&=\frac{2\overline{u}_*^4}{3}\int_{\overline{u}_*^3}^{1}\frac{dt}{t^{4/3}\sqrt{t^2-\overline{u}_*^6}}\left(1+\frac{\alpha^4t^{4/3}}{2}-\frac{\alpha^8t^{8/3}}{8}+\dots\right)\\
%     lu_*&=\left[\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}-\frac{1}{2} \overline{u}_*^4 \, _2F_1\left(\frac{1}{2},\frac{2}{3};\frac{5}{3};\overline{u}_*^6\right)\right]+\left[\frac{1}{6} \alpha ^4 \overline{u}_*^4 \log \left(\frac{1+\sqrt{1-\overline{u}_*^6}}{1-\sqrt{1-\overline{u}_*^6}}\right)\right]\label{exactluStar}\\ 
%     &\hspace{2cm}-\left[\frac{1}{48} \alpha ^8 \overline{u}_*^4 \left(3 \, _2F_1\left(-\frac{2}{3},\frac{1}{2};\frac{1}{3};\overline{u}_*^6\right)+\frac{2 \sqrt{\pi } \overline{u}_*^4 \Gamma \left(-\frac{2}{3}\right)}{\Gamma \left(-\frac{1}{6}\right)}\right)\right]+\dots\nonumber\\
%     &=[b_0+f_1(\overline{u}_*)]+[\alpha^4f_2(\overline{u}_*)]+O[\alpha^8]
% \end{align}
% Here $b_0=\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}$  and $f_1(\overline{u}_*)=-\frac{1}{2} \overline{u}_*^4 \, _2F_1\left(\frac{1}{2},\frac{2}{3};\frac{5}{3};\overline{u}_*^6\right)$  and we can write $\overline{u}_*=\frac{l u_*}{l u_b}$ to substitute in (\ref{exactluStar}) and expand in appropriate orders to get $u_*$ in terms of $l$ until first order in $\alpha^4$ as follows. The $\overline{u}_*$ in $f_1$ must be expanded until the $\alpha^4$ order,
% \begin{align}
%     lu_*&=b_0+f_1\left(\frac{lu_*}{lu_b}\right)+\alpha^4f_2\left(\frac{lu_*}{lu_b}\right)+O[\alpha^8]\\
%     &=b_0+f_1\left(\frac{b_0+f_1(\overline{u}_*)+\alpha^4 f_2(\overline{u}_*)}{lu_b}\right)+\alpha^4f_2\left(\frac{b_0+f_1(\overline{u}_*)}{lu_b}\right)+O[\alpha^8]\\
%     &=b_0+f_1\left(\frac{b_0+f_1(b_0+f_1(\overline{u}_*)/lu_b)+\alpha^4 f_2(b_0+f_1(\overline{u}_*)/lu_b)}{lu_b}\right)+\alpha^4f_2\left(\frac{b_0+f_1(b_0+f_1(\overline{u}_*)/lu_b)}{lu_b}\right)+O[\alpha^8]
% \end{align}
% This leads to a infinite cascade of terms as the $\alpha^0$ coefficient is not a constant, but rather it is a function of $\overline{u}_*$. So it is better if we take the series expansion of $\overline{u}_*$ near $0$ and this would give the $\alpha^0$ coefficient as a constant i.e. $f_1(\overline{u}_*)=0$. This would give,
% {\color{blue}Presumably the RHS in the line above is exact in $\overline{u}_*$, and only been expanded in powers of $\alpha$. Then one can and should invert it to be obtain $u_*$ as a function of $l$ here itself. One can defer expansion in $\overline{u}_*$ for a later stage for the two cases.}
% \begin{align}
%     lu_*&=\left[\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}-\frac{1}{2} \overline{u}_*^4(1+O[\overline{u}_*^6])\right]+\left[\frac{1}{6} \alpha^4 \overline{u}_*^4 \log \left(\frac{4}{\overline{u}_*^6}\right)+O\left(\overline{u}_*^6\right)\right]-\frac{1}{48} \alpha ^8 \overline{u}_*^4 \left(\frac{2 \sqrt{\pi } \overline{u}_*^4 \Gamma \left(-\frac{2}{3}\right)}{\Gamma \left(-\frac{1}{6}\right)}+3(1+O[\overline{u}_*^6])\right)+\dots\\
%     lu_*&=\left[\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}\right]+\left[\frac{1}{6} \alpha^4 \overline{u}_*^4 \log \left(\frac{4}{\overline{u}_*^6}\right)\right]-\frac{1}{48} \alpha ^8 \overline{u}_*^4 \left(\frac{2 \sqrt{\pi } \overline{u}_*^4 \Gamma \left(-\frac{2}{3}\right)}{\Gamma \left(-\frac{1}{6}\right)}+3\right)+\dots\label{luStarads}\\
%     u_*&=\frac{1}{l}\left(b_0+\alpha^4g_1(\overline{u}_*)+\alpha^8g_2(\overline{u}_*)+\dots\right)
% \end{align}
% Where $b_0=\frac{2\sqrt{\pi} \Gamma \left(\frac{2}{3}\right)}{\Gamma \left(\frac{1}{6}\right)}$, $g_1(\overline{u}_*)=\frac{1}{6}\overline{u}_*^4 \log \left(\frac{4}{\overline{u}_*^6}\right)$. Here we can write $\overline{u}_*=\frac{l u_*}{l u_b}$ and use (\ref{luStarads}) to substitute in $\bar{u}_$ and expand in appropriate orders to get $u_*$ in terms of $l$ until first order in $\alpha^4$ as follows,
% \begin{align}
%     u_*&=\frac{1}{l}\left(b_0+\alpha^4f_1\left(\frac{lu_*}{lu_b}\right)+\dots\right)=\frac{1}{l}\left(b_0+\alpha^4f_1\left(\frac{b_0}{lu_b}\right)+\dots\right)\\
%     u_*&=\frac{1}{l}\left(b_0+\frac{\alpha^4}{6}\left(\frac{b_0}{(u_b l)}\right)^4Log\left(\frac{4u_b^6l^6}{b_0^6}\right)+O[\alpha^8]\right)\\
%     u_*&=\frac{2 \sqrt{\pi } \Gamma \left(\frac{2}{3}\right)}{l\Gamma \left(\frac{1}{6}\right)}-\frac{a^4}{l^5}\frac{8 \pi ^2  \Gamma \left(\frac{2}{3}\right)^4}{3  \Gamma \left(\frac{1}{6}\right)^4} \left(6 \log \left(\frac{\Gamma \left(\frac{2}{3}\right)}{l u_b \Gamma \left(\frac{1}{6}\right)}\right)+\log \left(16 \pi ^3\right)\right)
% \end{align}

% {\color{blue} The RHS of the equation above should be massaged into the form,
% \begin{equation*}
%  u_* = \frac{b_0}{l} \left(1+ \alpha\,f_1\left(\frac{u_*}{u_B}\right) +\alpha^2\,f_2\left(\frac{u_*}{u_B}\right) + \ldots \right)
% \end{equation*}
% where $f_1,f_2$ are known functions. Then plug in this expansion of the $l\,u_*$ in each of the arguments of $f_1,f_2$ in the RHS of the equality above and expand each of those functions in $\alpha$ which in the end will lead to a solution of the form,
% \begin{equation*}
%     u_*= \frac{c_0}{l} \left(1+ \alpha\,g_1\left(\frac{1}{l\,u_B}\right)+ \alpha^2\,g_2\left(\frac{1}{l\,u_B}\right) +\ldots\right).
% \end{equation*}
% in the RHS where $g_1,g_2$ are functions of $1/(l\,u_B)$) which are to be determined in the process.
% \\
% \\}
% So we now write $u_*$ in term of $l$ by solving perturbatively in $\epsilon=a^4$. we first take the ansatz as $u_*=u_{*0}+(a^4 u_{*1})+(a^8 u_{*2})+\dots$. We get,
% \begin{align}
%     u_{*0}=\frac{\Gamma \left(\frac{2}{3}\right) \Gamma \left(\frac{5}{6}\right)}{\sqrt{\pi } l}\quad u_{*1}=\frac{a^4 \Gamma \left(\frac{2}{3}\right)^4 \Gamma \left(\frac{5}{6}\right)^4 \log \left(\frac{4 \pi ^3 l^6 u_B^6}{\Gamma \left(\frac{2}{3}\right)^6 \Gamma \left(\frac{5}{6}\right)^6}\right)}{6 \pi ^2 l^5}\\
% \end{align}
% So the $u_*$ is given as,
% \begin{align}\label{uStarinlads}
%     u_*=\frac{\Gamma \left(\frac{2}{3}\right) \Gamma \left(\frac{5}{6}\right)}{\sqrt{\pi } l}+\frac{a^4 \Gamma \left(\frac{2}{3}\right)^4 \Gamma \left(\frac{5}{6}\right)^4}{l^56 \pi ^2 } \log \left(\frac{4 \pi ^3 l^6 u_B^6}{\Gamma \left(\frac{2}{3}\right)^6 \Gamma \left(\frac{5}{6}\right)^6}\right)+O[a^8]
% \end{align}
\subsubsection{Far from AdS expansion}
 In the previous subsection we saw how $u_*$ can be expanded in the near AdS limit. Now we write $u_*$ in terms of $l$ when $\overline{a}>>1$ i.e. far from AdS. 
\begin{align}
    \sqrt{1+(\overline{a} x)^4}=(\overline{a} x)^2\sqrt{1+\frac{1}{(\overline{a} x)^4}}=\overline{a}^2x^2\left(1+\frac{1}{2\overline{a}^4 x^4}+\dots\right).
\end{align} 
Using this we have,
\begin{align}
    1&=2x_*^3\int_{x_*}^{x_b}\frac{dx\sqrt{1+\bar{a}^4 x^4}}{x^2\sqrt{x^6-x_*^6}}\\
    x_*&=2x_*^4\int_{x_*}^{x_b}\frac{dx\sqrt{1+\bar{a}^4 x^4}}{x^2\sqrt{x^6-x_*^6}}\\
    x_*&=2x_*^4\int_{x_*}^{x_b}\frac{dx\  \overline{a}^2x^2}{x^2\sqrt{x^6-x_*^6}}\left(1+\frac{1}{2\overline{a}^4 x^4}+\dots\right)\\
    x_*&= -\frac{2 \sqrt{\pi } \overline{a}^2 x_*^2 \Gamma \left(\frac{1}{3}\right)}{\Gamma \left(-\frac{1}{6}\right)}+O\left(\frac{1}{\overline{a}^2}\right)\\
    x_*&\sim -\frac{2 \sqrt{\pi } \overline{a}^2 x_*^2 \Gamma \left(\frac{1}{3}\right)}{\Gamma \left(-\frac{1}{6}\right)}\\
    x_*&\sim -\frac{\Gamma(-\frac{1}{6})}{2\sqrt{\pi}\overline{a}^2 \Gamma(\frac{1}{3})}\label{uStarinlfarads}\\
    u_*&\sim \frac{l}{a^2}\frac{\Gamma(\frac{5}{6})}{2\sqrt{\pi} \Gamma(\frac{4}{3})}
\end{align}
Now we find the critical length, at which transiion happens, by finding the limiting case of far from AdS case as,
\begin{align}
    l&=2 u_*^3 \int_{u_*}^{\infty}du\  \frac{a^2}{\sqrt{u^6-u_*^6}}\left(1+\frac{1}{2a^4u^4}+O\left(\frac{1}{a^8}\right)\right)\\
    &=\frac{a^2 u_* \sqrt{\pi}\Gamma\left(\frac{1}{3}\right)}{3\Gamma\left(\frac{5}{6}\right)}-\frac{1}{3 a^2 u_*^3}+O\left(\frac{1}{a^4}\right)
\end{align}
To above length is dependent on $u_*$, which can be found by finding the derivative of $l$ w.r.t. $u_*$ and equating this to zero as this is the turning point. Here we redefine everything with $u_*$ by taking $u/u_*=t^{1/3}$ and $\bar{a}=a u_*$,
\begin{align}
    l&=2 u_*^3\int_{u_*}^{\infty}du\ \frac{\sqrt{1+a^4u^4}}{u^2(x)\sqrt{u^6(x)-u_*^6}}\\
    \frac{dl}{du_*}&=-\frac{2}{u_*}\int_1^{\infty}dt \ \frac{1+\bar{a}^4t^4}{t^2\sqrt{t^2-1}}+4a^4u_*^2\int_1^{\infty}dt\ \frac{t^2}{\sqrt{t^2-1}\sqrt{1+\bar{a}^4 t^4}}=0\\
    \implies \frac{2}{u_*}\int_1^{\infty}dt \ \frac{1+\bar{a}^4t^4}{t^2\sqrt{t^2-1}}&=4a^4u_*^2\int_1^{\infty}dt\ \frac{t^2}{\sqrt{t^2-1}\sqrt{1+\bar{a}^4 t^4}}\\
    2\bar{a}^4&=\left(\int_1^{\infty}\frac{\sqrt{1+\bar{a}^4t^4}}{t^2\sqrt{t^2-1}}\right)/\left(\int_1^{\infty}dt \ \frac{t^2}{\sqrt{t^2-1}\sqrt{1+\bar{a}^4t^4}}\right)\\
    2\bar{a}^4&\sim \bar{a}^4-\frac{\Gamma \left(-\frac{1}{6}\right)}{9 \sqrt{\pi } \Gamma \left(\frac{4}{3}\right)}\\
    u_*&\sim\frac{2\Gamma\left(\frac{5}{6}\right)}{a \sqrt{\pi}\Gamma\left(\frac{1}{3}\right)}\\
    l_{\text{critical}}&\sim \frac{a \ \sqrt{3} \Gamma \left(\frac{1}{3}\right) \Gamma \left(\frac{7}{6}\right)^{3/4}}{2^{3/4} \pi ^{3/8} \sqrt[4]{\Gamma \left(\frac{4}{3}\right)}}\\
    \implies l_{\text{critical}}&\sim 1.74 a
\end{align}
\begin{table}[H]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    a & Analytical value & Value from Plot\\
    \hline
    $10^{-7}$&  $1.74\cdot 10^{-7}$ & $1.64\cdot 10^{-7}$\\
    \hline
    $10^{-5}$& $1.7\cdot 10^{-5}$   & $1.6\cdot 10^{-5}$\\
    \hline
    $10^{-3}$& 0.0017  &0.0016\\
    \hline
    $10^{-1}$&  0.17 &0.17\\ 
    \hline
    \end{tabular}
\end{table}
In all the plots we have $u_B=10^{8}$ and $a=10^{-7}$, until and unless mentioned. The graph of function of pure AdS $l_0$ and $l$ vs $u_*$ are given as,
\begin{figure}[H]
    \centering
     \includegraphics[width=0.5\linewidth]{images_volume_complexity/lAdsvsuStar.jpg}\hfill
    \includegraphics[width=0.5\linewidth]{images_volume_complexity/lvsuStar_f.jpg}
    \caption{$l_0$(a=0) vs $u_*$ and $l(a\neq0)$ vs $u_*$}
    \label{fig:enter-label}
\end{figure}

\subsection{Sub region volume complexity-Non-isotropic case}
Now we want to compute the sub region complexity given by the co-dimension 1 surface given by,
\begin{align}
    ds^2&=R^2 u^2(h(u)(dx^2+dy^2)+dz^2)+R^2\frac{du^2}{u^2}+R^2d\Omega^2_5\
\end{align}
The volume is given by,
\begin{align}
    V&=\int e^{-2(\phi-\phi_0)} \sqrt{|\tilde{g}_{\mu\nu}|}d^Dx\\
    &=\int e^{-2(\phi-\phi_0)}\sqrt{R^{10} u^4h^2(u)}dx\ dy\ dz\ du\\
    &=R^9\omega_5\int_{-W/2}^{W/2}dy\int_{-W/2}^{W/2}dz\int_{u_*}^{u_B}du\int_{0}^X u^2h(u)e^{-2(\phi-\phi_0)}dx\\
    &=R^9\omega_5\int_{-W/2}^{W/2}dy\int_{-W/2}^{W/2}dz\int_{u_*}^{u_B}du u^2(x)\int_{0}^X dx\\
    &=2R^9\omega_5\int_{-W/2}^{W/2}dy\int_{-W/2}^{W/2}dz\int_{u_*}^{u_B}du u^2(x)\int_{u_*}^{u_B} \frac{d\tilde{u}}{{\tilde{u}^2}\sqrt{h(\tilde{u})}\sqrt{\tilde{u}^6-u_*^6}}\\
    V&=R^9W^2\omega_5 (2u_*^3)\int_{u_*}^{u_B}du u^2(x)\int_{u_*}^{u_B} \frac{d\tilde{u}}{{\tilde{u}^2}\sqrt{h(\tilde{u})}\sqrt{\tilde{u}^6-u_*^6}}
\end{align}
We now use the numerical integration to plot the complexity $V(u_*,u_B)$ vs $l(u_*)$. We get the plot for $V(u_*)$ vs $l(u_*)$ and $Log(V(u_*))$ vs $l(u_*)$ as follows Figure 2.\\
\begin{figure}[H]
    \centering
    \includegraphics[width=7cm,height=6cm]{images_volume_complexity/Vvsl_a10-7_f.jpg}\hfill
    \includegraphics[width=7cm,height=6cm]{images_volume_complexity/LogVvsLogl_a10-7_f.jpg}
    \caption{ V vs l and Log[V] vs Log[l]}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=7cm,height=6cm]{images_volume_complexity/LogVvsLogl_a10-5_f.jpg}\hfill
    \includegraphics[width=7cm,height=6cm]{images_volume_complexity/LogVvsLogl_a10-3_f.jpg}\hfill
    \caption{Here to left $a=10^{-5}$ and to right$a=10^{-3}$}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=7cm,height=6cm]{images_volume_complexity/LogVvsLogl_a10-1_f.jpg}\hfill
    \includegraphics[width=7cm,height=6cm]{images_volume_complexity/LogVvsLogl_Comp.jpg}
    \caption{Here $a=10^{-1}$}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=7cm,height=6cm]{images_volume_complexity/LogVvsLogl_a10-9_f.jpg}\hfill
    \includegraphics[width=7cm,height=6cm]{images_volume_complexity/LogVvsLogl_a10-11_f.jpg}\hfill
    \caption{Here to left $a=10^{-9}$ and to right $a=10^{-11}$}
    \label{fig:enter-label}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=7cm,height=6cm]{images_volume_complexity/LogVvsLogl_a10-13_f.jpg}\hfill
    \includegraphics[width=7cm,height=6cm]{images_volume_complexity/LogVvsLogl_a10-15_f.jpg}\hfill
    \caption{Here to left $a=10^{-13}$ and to right $a=10^{-15}$}
    \label{fig:enter-label}
\end{figure}
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.5\linewidth]{images_volume_complexity/logVvslogl_a10-8.jpg}\hfill
%     \caption{Log[V] vs Log[l] graph. Here $a=10^{-8}$}
%     \label{fig:enter-label}
% \end{figure}
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.5\linewidth]{logvvslogl_differenta.jpg}
%     \caption{Graph for different a}
%     \label{fig:enter-label}
% \end{figure}
\noindent From Fig. 1 and Fig. 2, we can see that the transition point is same in both $l$ vs $u_*$ and $V$ vs $l$ graphs. The transition point is given as $(u_{*tran},l_{tran})=(8*10^6,1.6*10^{-7})$ and similarly in $V$ vs $l$, we have the transition point as $(l_{tran},V_{tran})=(1.6*10^{-7},2.7*10^{16}$. Until now we have $a=10^{-7}$, but now we will plot Log$[V]$ vs Log$[l]$ for different values of $a$, as shown in Fig. 3-6.
\subsubsection{Near AdS regime}

Here as well we have two different regions which is near AdS and far from AdS and we substitute the appropriate $u_*$ to get the analytical result of $C_V$ in terms of l until the first order. Here we first convert the integrads into dimensionless quantities, $\overline{a},x_*, x_b$.
\begin{align}
    V&=R^4W^2 (2u_*^3)\int_{u_*}^{u_B}du u^2(x)\int_{u_*}^{u_B} \frac{d\tilde{u}}{{\tilde{u}^2}\sqrt{h(\tilde{u})}\sqrt{\tilde{u}^6-u_*^6}}\\
    &=R^4W^2  \frac{2x_*^3}{l^2}\int_{x_*}^{x_b} x^2 dx\int_{x_*}^{x}\frac{\sqrt{1+\overline{a}^4 \tilde{x}^4}}{\tilde{x}^2\sqrt{\tilde{x}^6-x_*^6}}\\
    &=R^4W^2  \frac{2x_*^3}{l^2}\int_{x_*}^{x_b} x^2 dx\int_{x_*}^{x}\frac{1}{\tilde{x}^2\sqrt{\tilde{x}^6-x_*^6}}\left(1+\frac{\overline{a}^4 x^4}{2}-\frac{\overline{a}^8 x^8}{8}+O(a^{12})\right)\\
    &=R^4W^2\left(\frac{\sqrt{\pi }}{81 l^2 x_*} \left(\frac{2 \sqrt{3} \pi  x_b^3}{\Gamma \left(\frac{7}{6}\right) \Gamma \left(\frac{4}{3}\right)}-\frac{9 x_*^3 \Gamma \left(\frac{1}{6}\right)}{\Gamma \left(\frac{2}{3}\right)}\right)+\frac{\overline{a}^4 x_b^3 x_*^3}{9 l^2} \left(-3 \log \left(\frac{x_*}{\sqrt[3]{2} x_b}\right)-1\right)+O(\overline{a}^8)\right)\\
    &=R^4W^2\left(\frac{\sqrt{\pi }}{81 u_*} \left(\frac{2 \sqrt{3} \pi  u_b^3}{\Gamma \left(\frac{7}{6}\right) \Gamma \left(\frac{4}{3}\right)}-\frac{9 u_*^3 \Gamma \left(\frac{1}{6}\right)}{\Gamma \left(\frac{2}{3}\right)}\right)+\frac{1}{9} a^4 u_b^3 u_*^3 \left(-3 \log \left(\frac{u_*}{\sqrt[3]{2} u_b}\right)-1\right)+O(a^8)\right)\\
    &=R^4W^2\left(\frac{\sqrt{\pi }}{81}\left(\frac{1}{u_{00}}-\frac{a^4 u_{11}}{u_{00}^2}\right) \left(\frac{2 \sqrt{3} \pi  u_b^3}{\Gamma \left(\frac{7}{6}\right) \Gamma \left(\frac{4}{3}\right)}-\frac{9 u_*^3 \Gamma \left(\frac{1}{6}\right)}{\Gamma \left(\frac{2}{3}\right)}\right)+\frac{1}{9} a^4 u_b^3 u_*^3 \left(-3 \log \left(\frac{u_*}{\sqrt[3]{2} u_b}\right)-1\right)+O(a^8)\right)
\end{align}
Here we took the expansion of $1/u_*$ in the first term until first order in $\epsilon=\alpha^4$. Now we substitute eq.(\ref{uStarinlnearads}) to write $V$ in terms of $l$ as,
\begin{align}
   V&=R^4 W^2\left(\frac{l u_b^3}{3}-\frac{4 \pi ^{3/2} \Gamma \left(\frac{2}{3}\right)}{9 l^2 \Gamma \left(\frac{1}{6}\right)}+a^4 \left(\frac{128 \pi ^{9/2} \Gamma \left(\frac{2}{3}\right)^9}{9 l^9 u_b^3 \Gamma \left(\frac{1}{6}\right)^9}-\frac{8 \pi ^{3/2} u_b^3 \Gamma \left(\frac{2}{3}\right)^3}{9 l^3 \Gamma \left(\frac{1}{6}\right)^3}\right)+O(a^8)\right)\\
   C_V&=\frac{R^3 W^2}{G_N^{(5)}}\left(\frac{l u_b^3}{3}-\frac{4 \pi ^{3/2} \Gamma \left(\frac{2}{3}\right)}{9 l^2 \Gamma \left(\frac{1}{6}\right)}+a^4 \left(\frac{128 \pi ^{9/2} \Gamma \left(\frac{2}{3}\right)^9}{9 l^9 u_b^3 \Gamma \left(\frac{1}{6}\right)^9}-\frac{8 \pi ^{3/2} u_b^3 \Gamma \left(\frac{2}{3}\right)^3}{9 l^3 \Gamma \left(\frac{1}{6}\right)^3}\right)+O(a^8)\right)
\end{align}
If we take the pure AdS case $a=0$ in the above case, we have eq.(\ref{Vpureads}). This exactly matches with the eq.2.11 from \href{https://arxiv.org/pdf/1609.02514}{Ami, Carmi}.
\begin{align}
    V_0(pure \ AdS)=R^4W^2\left(\frac{l u_B^3}{3}-\frac{4 \pi ^{3/2} \Gamma \left(\frac{2}{3}\right)}{9 l^2 \Gamma \left(\frac{1}{6}\right)}\right)\label{Vpureads}\\
    C_V=\frac{R^3W^2}{G_N^{(5)}}\left(\frac{l u_B^3}{3}-\frac{4 \pi ^{3/2} \Gamma \left(\frac{2}{3}\right)}{9 l^2 \Gamma \left(\frac{1}{6}\right)}\right)\label{Vpureads}
\end{align}
\subsubsection{Far from AdS regime}
We would also have two other cases in which $a>>l>>1/u_B$ and $l>>a>>1/u_B$. In both of these $\bar{a}=au_B>>1$ so we take this limit first. We use eq.(\ref{uStarinlfarads}) and write V in terms of $l$.
\begin{align}
    V&=R^4W^2 (2u_*^3)\int_{u_*}^{u_B}du u^2(x)\int_{u_*}^{u} \frac{d\tilde{u}}{{\tilde{u}^2}\sqrt{h(\tilde{u})}\sqrt{\tilde{u}^6-u_*^6}}\\
    &=R^4W^2  \frac{2x_*^3}{l^2}\int_{x_*}^{x_b} x^2 dx\int_{x_*}^{x}d\tilde{x}\frac{\sqrt{1+\overline{a}^4 \tilde{x}^4}}{\tilde{x}^2\sqrt{\tilde{x}^6-x_*^6}}\\
    &=R^4W^2  \frac{2x_*^3}{l^2}\int_{x_*}^{x_b} x^2 dx\int_{x_*}^{x}d\tilde{x}\frac{\overline{a}^2}{\sqrt{\tilde{x}^6-x_*^6}}\left(1+\frac{1}{2\overline{a}^4x^4}-\frac{1}{8 \overline{a}^8 u^8}+O\left(\frac{1}{\overline{a}^{12}}\right)\right)\\
    &\sim R^4W^2  \frac{2x_* \overline{a}^2}{3 l^2}\int_{x_*}^{x_b} x^2 dx\int_{1}^{(x/x_*)^3}d\tilde{x}\ \frac{1}{t^{2/3}\sqrt{\tilde{t}^2-1}}\\
    &\sim R^4W^2  \frac{2x_* \overline{a}^2}{3 l^2}\int_{x_*}^{x_b} x^2 dx\int_{1}^{(x/x_*)^3}d\tilde{x}\ \frac{\overline{a}^2}{t^{2/3}\sqrt{\tilde{t}^2-1}}\\
    &\sim R^4W^2 \left(-\frac{2 \sqrt{\pi } \overline{a}^2 x_b^3 x_* \Gamma \left(\frac{1}{3}\right)}{3 l^2 \Gamma \left(-\frac{1}{6}\right)}-\frac{\overline{a}^2 x_b x_*^3}{l^2}+\frac{\overline{a}^2 x_* \left(\frac{6 \sqrt{\pi } x_*^3 \Gamma \left(\frac{1}{3}\right)}{\Gamma \left(-\frac{1}{6}\right)}-\frac{\sqrt{\pi } x_*^3 \left(-\frac{2 \Gamma \left(\frac{5}{6}\right)^2}{\Gamma \left(\frac{4}{3}\right)}-\Gamma \left(\frac{1}{3}\right)\right)}{\Gamma \left(\frac{5}{6}\right)}\right)}{9 l^2}\right)
\end{align}
Now we substitute eq. (\ref{uStarinlfarads}) to write the Volume in terms of $l$ as follows,
\begin{align}
    V&\sim R^4W^2\left( \frac{l u_b^3}{3}-\frac{l^3 u_b}{a^4}\frac{ \Gamma \left(-\frac{1}{6}\right)^4}{32 \sqrt[3]{2} \sqrt{3} \pi ^3 \Gamma \left(\frac{1}{3}\right)}+\frac{l^4}{a^6}\frac{\sqrt{3} \Gamma \left(\frac{5}{6}\right)^6}{\sqrt[3]{2} \pi ^3\Gamma \left(\frac{4}{3}\right)^3}\right)\\
    C_V&=\frac{R^3}{G_N^{(5)}}\left(\frac{W^2l u_b^3}{3}+\frac{W^2l^4}{a^6}\frac{\sqrt{3} \Gamma \left(\frac{5}{6}\right)^6}{\sqrt[3]{2} \pi ^3\Gamma \left(\frac{4}{3}\right)^3}-\frac{W^2l^3 u_b}{a^4}\frac{ \Gamma \left(-\frac{1}{6}\right)^4}{32 \sqrt[3]{2} \sqrt{3} \pi ^3 \Gamma \left(\frac{1}{3}\right)}\right)
\end{align}
We plot these analytical solutions and see whether they match the numerical solution as given in the Figure 7.
% We can find the knee points for the plots in Fig.3 and Fig.4 using the above formula as follows,
% \begin{center}
% \begin{tabular}{ |c|c|c|} 
%   \hline
%   a&  From plot  & Value from above formula\\ 
%   \hline
%   $10^{-7}$& $1.37\cdot 10^{17}$ & $1.382\cdot 10^{17}$\\ 
%   \hline
%   $10^{-6}$& -&- \\ 
%   \hline
%    $10^{-5}$& -&- \\
%    \hline
%     $10^{-3}$& -& - \\
%    \hline
%    $10^{-1}$& -& -\\
%    \hline
%    \end{tabular}
% \end{center}


 \begin{multicols}{2}
        \begin{figure*}[ht!]
            \includegraphics[width=.35\textwidth]{images_volume_complexity/Vvsl_-7_Comp.jpg}\hfill
            \includegraphics[width=.35\textwidth]{images_volume_complexity/LogVvsLogl_-7_Comp.jpg}\hfill
            % \includegraphics[width=.3\textwidth]{images_volume_complexity/LogVvsLogl_aminus5_comp.jpg}
        \caption{Here $a=10^{-7}$. From the above plot we can see that the analytical expressions closely match the numerical plot in the respective regimes. The AdS region is to the right half of the plots and the far from AdS region is towards the left half of the plot.}
        \end{figure*}
    \end{multicols}

% Now we will see that graphically as to what extent $V$ and $V_0$ are valid. The plots of $V$ and $V_0$ are as follows,
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=6cm,height=6cm]{images_volume_complexity/LogVvsLogl_nonAdS.jpg}\hfill
%     \includegraphics[width=6cm,height=6cm]{images_volume_complexity/LogVvsLogl_AdS.jpg}
%     \caption{Left side is for $au_B>>1$ and right side is for $au_B<<1$}
%     \label{fig:enter-label}
% \end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=7cm,height=7cm]{images_volume_complexity/Combined_V0_V_VNIntegration.jpg}
    \caption{Combined graph when $au_B>>1$ given by red dots and $au_B<<1$ given by green dots and blue line is when we do numerical integration without taking any limits. We see that green dots can be used in the AdS limit and Red dotted line is used for Non-AdS as expected.}
    \label{fig:enter-label}
\end{figure}
The above is when we keep $u_B$ fixed and change $a$. But now, we see what happens if we keep $a$ as constant and change $u_B$. Until now we have $a=10^{-7}$ and $u_B=10^{8}$. We will now keep $a=10^{-7}$ but change $u_B$, which would give the following plots,
\begin{figure}[H]
    \centering
    \includegraphics[width=0.4\linewidth]{images_volume_complexity/Vvsl_ub_different.jpg}
    \label{fig:enter-label}
\end{figure}
\subsection{Entanglement Entropy}
The entanglement entropy is given by eq. 48 as,
\begin{align}
    A&= R^8\omega_5\times W^2\times \int_{-l/2}^{l/2}u^3(x)\sqrt{1+\frac{(u'(x))^2}{u^4(x)h(u)}}dx
\end{align}
The graph of the entanglement entropy vs l is given as, which is also obtained in the paper \cite{Karczmarek:2013xxa}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{Avsl.jpg}
    \caption{graph of A vs l}
    \label{fig:enter-label}
\end{figure}











